UAV Trajectory and Multi-User Beamforming Optimization for Clustered Users Against Passive Eavesdropping Attacks With Unknown CSI

This paper tackles the fundamental passive eavesdropping problem in modern wireless communications in which the location and the channel state information (CSI) of the attackers are unknown. In this regard, we propose deploying an unmanned aerial vehicle (UAV) that serves as a mobile aerial relay (AR) to help ground base station (GBS) support a subset of vulnerable users. More precisely, our solution (1) clusters the single-antenna users in two groups to be either served by the GBS directly or via the AR, (2) employs optimal multi-user beamforming to the directly served users, and (3) optimizes the AR's 3D position, its multi-user beamforming matrix and transmit powers by combining closed-form solutions with machine learning techniques. Specifically, we design a plain beamforming and power optimization combined with a deep reinforcement learning (DRL) algorithm for an AR to optimize its trajectory for the security maximization of the served users. Numerical results show that the multi-user multiple input, single output (MU-MISO) system split between a GBS and an AR with optimized transmission parameters without knowledge of the eavesdropping channels achieves high secrecy capacities that scale well with increasing the number of users.

==> include/cluster.tex <==

The clustering problem here consists of %%K-means aims to 
dividing %a given set of $K$ data elements
the set $U$ of $K$ %deployed number of ground 
users %$\{u_1, u_2, \dots, u_K\}$ 
into the set $C$ of two %$R$ 
clusters. %% by %through
%%obtaining the %superior
%%cluster centers $\{c_1, c_2\}$. 





For solving the user clustering problem, we may %attempt to 
employ an exhaustive search, %which has shown a good performance for such scenarios, however, 
but it entails a high computational complexity, which increases exponentially with the number of users. %Therefore, in this paper we are going to utilize 
We instead apply K-means clustering, a %%learning-based algorithm for clustering users to be associated with the GBS or AR. %, %based on machine learning that 
%%The K-means algorithm is 
a popular unsupervised machine learning algorithm that is used for grouping a set of objects into different clusters so that the %based on the 
similarity criterion of cluster members is maximized. 
It takes any similarity metric %for calculating the  
and target number of clusters. It is a computationally efficient method when %has low-complexity
compared with other techniques such as graph theory, fuzzy c-means, and hierarchical clustering~\cite{clustering}. 

 %\textcolor{pink}{Is there always a single criterion?}
%clustering purpose
%The K-means clustering algorithm has been deployed in various communication networks scenarios, such as cognitive radio, spectrum sharing, resource allocation, traffic offloading, and interference/anomaly detection and classification \cite{VukVTC17}. 

%%The concept behind K-mean clustering is finding the centroids for a predefined number of clusters and assign each point to the nearest centroid to form a cluster. 
%%The ideal cluster centroids %achieved 
%%are the ones that guarantee the maximum similarity between the same cluster members and the maximum dissimilarity between the members of different clusters. 
%Based on the above description of the K-means working mechanism, 
%%Consequently, there are two main attributes that are critical for efficient clustering: the target number of clusters %that is pre-defined 
%%and the similarity metric. 
%%The K-means algorithm is applied in this paper to partition the ground users into two %different
%%clusters based on the quality of the G2G communication channel between the GBS and the users. More precisely, 
%\textcolor{cyan}{The clustering can be scaled to any number of clusters, for example when more than one GBS or more than one UAV are involved. }

%%The end goal of employing the K-means clustering algorithm is to determine the %cluster of 
%%users to be served by the GBS and those % other cluster where the users will 
%%to be served by the AR. 
%%We therefore %are going to 
%%define the normalized channel between the GBS and all users as

%\textcolor{pink}{formula here?} 

%\textcolor{pink}{is it between the GBS and each user or a single value combining all the K channels? for each user}

%the similarity metric. 
The normalized channel,

%of the normalized channel is given as follow 
\vspace{-10pt}
\begin{equation}
        h^n_{sk} = \frac{ h_{sk}}{\parallel h_{sk} \parallel_2},
    \label{eq:sim}
\vspace{-4pt}
\end{equation}
%$h^n$ is chosen 
covers the variations of channel gains resulting from different propagation factors, such as small-scale fading and shadow fading. %We define the similarity metric as
Parameter $h_{sk}$ is the channel gain between the GBS and user $k$ and $\parallel.\parallel_2$ is the $L_2$ vector norm.
The Euclidian distance is used to measure the similarity between the centroids of the clusters and %the other data points,
the normalized channels between the GBS and each UE to define the cluster members. %If the the Euclidian distance is selected normalized channel point as cluster center and the nominated points to be assigned as members within this centroid's cluster if the Euclidian distance is low compared with other centroids.   
The procedure %of K-means algorithm 
is as follows: First, the initial centroids $C=\{c_1, c_2\}$ are randomly selected as cluster centers %\hl{
from the available normalized channel data points $U=\{u_1, u_2, \dots, u_K\}$. %\textcolor{pink}{Don't understand what the last part means.} 
Second, the Euclidian distance between each normalized channel point and the cluster centers is calculated to assign the data points to the nearest centers. Next, the center of each cluster is updated to minimize the sum of squared Euclidean distance between the assigned users and their centroid. % for each cluster. 
Specifically, the following model is used to update the cluster centers: 
\vspace{-6pt}
\begin{equation}
       \min\limits_{C} \sum \limits_{k} \min\limits_{r\in R} \parallel h^n_{sk} - c_r  \parallel^2_2,
    \label{eq:K-meansCenterUpdate}
    \vspace{-7pt}
\end{equation}
where $C \triangleq \{c_r \mid r \in R\}$ and $R=2$ represents the number of clusters. 
After updating the cluster centers, the procedure of assigning ground users to the two clusters is repeated, after which %using the updated centroids. and after that the update of 
the centroids are %will be triggered 
recalculated. %again. 
This iterative process continues % user assignment and centrodis update steps are going to be repeated 
until no more changes occur on the centroids or the clusters. Algorithm~\ref{Algorithm1} illustrates the iterative procedure for %performing the K-means 
determining the two user clusters. Figure~\ref{fig:Clustering} shows an example clustering outcome based on this metric and algorithm. %%Note that the number or associated UEs per cluster is not necessarily balanced. %solution where the metric is the \hl{complex channel gain}.    
 \begin{minipage}{0.99\linewidth}
%  \begin{adjustwidth}{1em}{}
\SetKwRepeat{Do}{do}{while}%
 \begin{spacing}{1}
 \LinesNotNumbered
 \SetInd{1.15em}{0.5em}
\begin{algorithm}[H]
\footnotesize
\SetAlgoLined
\SetAlgoHangIndent{5.5em}
%\SetAlgoNoLine
%\setlength{\algomargin}{0pt}
%\begin{enumerate}[ itemsep=-10pt, topsep=2pt]
%\item 
    \phantom{.}\text{\bf{Input:}} $U$ and $C$\\
    \phantom{.}\text{\bf{Output:}} \ $K_c$ and $C$, $\forall \ c \in C $ \\
\phantom{....} \nl \text{\bf{Initialize}} \ \textit{cluster head set  $C_\mathcal{CH} = \emptyset$ and $c=1$}; \\ 

\vspace{-9 pt} \hspace{-6 pt}\nl  \Indp\While{c \ \leq \ C}{    
\phantom{....} \nl    \it{\hspace{-16 pt}Randomly select a cluster head $\mathcal{CH}_c$ from $U$;} \\
\phantom{....} \nl      \it{\hspace{-16 pt}Update $C_\mathcal{CH} =\{\mathcal{CH}_c, \forall \ c \in C$\};}\\
\phantom{....} \nl         \hspace{-16 pt}c = c + 1;\\\vspace{-7 pt}}
\phantom{....-}\nl     \hspace{-18 pt} \Repeat{ \hspace{+4 pt}\it{The cluster members do not change}}
{ 
\phantom{...-} \nl         \it{\multiline{\hspace{-16 pt}For each user $m \in U$, calculate the minimum Euclidean distance \\\hspace{-16 pt}from the $\mathcal{CH}_c$;}}\\
\phantom{....} \nl         \it{\hspace{-16 pt}Fit each user to the closest cluster;}\\
\phantom{...-} \nl         \it{\multiline{\hspace{-16 pt}Update  the cluster head $\mathcal{CH}_c$ by taking the average of all \\\hspace{-16 pt}the users $m$; }}}
%\nl         \bf{until} \it{The cluster members do not change}\\
\caption{\small K-means user clustering in MU-MISO environment.}
\label{Algorithm1}
\end{algorithm}
  \end{spacing}
% \end{adjustwidth}
\end{minipage}

\begin{figure}[ht]
%\vspace{-24 pt}
	   \centering
	   \includegraphics[width=0.50\textwidth]{figures/UAVC/Clustering2.eps}
	    %\vspace{-9 pt}
        \caption{Channel-based clustering. %\hl{optional, can go if we do not have space} %\hl{Vuk: Would it make sense to also provide the other two clustering results (Fig. 4a, b, c) and label the UEs in the plot, e.g. from 1 to 16, so we can get an idea how their cluster association changes depending on the metric used? For now, let's keep just this example and relocate it}
        }
        %\vspace{-3 mm}
        \label{fig:Clustering}
\end{figure}

\textcolor{cyan}{%K-means clustering 
Algorithm 1 can apply any similarity metric. Several other options exist here, such as distance based clustering or rate based clustering, where UEs with the nearest distance to the GBS and the highest downlink rates, respectively, may be grouped. % into one cluster. %, and channel base clustering. %, and eavesdropper rate base clustering. 
%Based on the similarity of the values according to the chosen metric, the K-means clustering places the UEs two clusters. %in this case. 
The metric can have an effect on the system performance and should be chosen based on the objective and the ability or simplicity to obtain the necessary information to calculate the value for each UE, which may require feedback from the UE %, eavesdropper, 
or other nodes in the network.  %Other options include distance or \hl{rate based} clustering with respect to the GBS, for instance. 
}



==> include/cluster_new.tex <==


\color{black}
The goal of user clustering is to divide $K$ users into two clusters, one cluster is to be served by the GBS and the other cluster is served the UAV.
\color{black}




% The clustering problem here consists of 
% dividing %a given set of $K$ data elements
% the set %$U$ 
% of $K$ %deployed number of ground 
% users %$\{u_1, u_2, \dots, u_K\}$ 
% into the set %$C$ 
% of two %$R$ 
% clusters. %% by %through
% %%obtaining the %superior
%%cluster centers $\{c_1, c_2\}$. 



For solving the user clustering problem, we can employ an exhaustive search, but it entails a high computational complexity, which increases exponentially with the number of users. We instead apply K-means clustering, a unsupervised machine learning algorithm that is used for grouping a set of objects so that the similarity criterion of members in a group and the dissimilarity with members of other groups is maximized. 
K-mean works with any single or multi-dimensional metric that the data captures and user-defined target number of clusters \cite{VukVTC17}. It is a computationally efficient method  compared to other techniques such as graph theory, fuzzy c-means clustering, and hierarchical clustering~\cite{clustering}. 

 %\textcolor{pink}{Is there always a single criterion?}
%clustering purpose
%The K-means clustering algorithm has been deployed in various communication networks scenarios, such as cognitive radio, spectrum sharing, resource allocation, traffic offloading, and interference/anomaly detection and classification \cite{VukVTC17}. 

%%The concept behind K-mean clustering is finding the centroids for a predefined number of clusters and assign each point to the nearest centroid to form a cluster. 
%%The ideal cluster centroids %achieved 
%%are the ones that guarantee the maximum similarity between the same cluster members and the maximum dissimilarity between the members of different clusters. 
%Based on the above description of the K-means working mechanism, 
%%Consequently, there are two main attributes that are critical for efficient clustering: the target number of clusters %that is pre-defined 
%%and the similarity metric. 
%%The K-means algorithm is applied in this paper to partition the ground users into two %different
%%clusters based on the quality of the G2G communication channel between the GBS and the users. More precisely, 
%\textcolor{cyan}{The clustering can be scaled to any number of clusters, for example when more than one GBS or more than one UAV are involved. }

%%The end goal of employing the K-means clustering algorithm is to determine the %cluster of 
%%users to be served by the GBS and those % other cluster where the users will 
%%to be served by the AR. 
%%We therefore %are going to 
%%define the normalized channel between the GBS and all users as

%\textcolor{pink}{formula here?} 

%\textcolor{pink}{is it between the GBS and each user or a single value combining all the K channels? for each user}

%the similarity metric. 

The Euclidian distance is used to measure the similarity between the centroids, or cluster centers, %of the two clusters and %the other data points,
and the UE-specific data points to determine the cluster association. %If the the Euclidian distance is selected normalized channel point as cluster center and the nominated points to be assigned as members within this centroid's cluster if the Euclidian distance is low compared with other centroids.   
The procedure %of K-means algorithm 
is as follows: First, the initial centroids $C=\{c_1, c_2\}$ are randomly selected as cluster centers %\hl{
from the $K$ available %normalized channel 
data points: $U=\{u_1, u_2, \dots, u_K\}$. %\textcolor{pink}{Don't understand what the last part means.} 
Second, the Euclidian distance between each data point and the cluster centers is calculated to assign the data point to the nearest center. Next, the centroids are updated to minimize the sum of squared Euclidean distances between a user and its centroid, % for each cluster. 
%The following model is used to update the cluster centers: 
\vspace{-5pt}
\begin{equation}
       \min\limits_{C} \sum \limits_{k} \min\limits_{r\in R} \parallel u_{k} - c_r  \parallel^2_2,
    \label{eq:K-meansCenterUpdate}
    \vspace{-7pt}
\end{equation}
where $C \triangleq \{c_r \mid r \in R\}$ and $R=2$ represents the number of clusters. 
After updating the cluster centers, the procedure of assigning users to the two clusters is repeated, after which %using the updated centroids. and after that the update of 
the centroids are %will be triggered 
recalculated. %again. 
This iterative process continues % user assignment and centrodis update steps are going to be repeated 
until no more changes occur to the centroids and cluster association. Algorithm~\ref{Algorithm1} illustrates the iterative procedure for %performing the K-means 
determining the two user clusters.    
 \begin{minipage}{0.99\linewidth}
%  \begin{adjustwidth}{1em}{}
\SetKwRepeat{Do}{do}{while}%
 \begin{spacing}{1}
 \LinesNotNumbered
 \SetInd{1.15em}{0.5em}
\begin{algorithm}[H]
\footnotesize
\SetAlgoLined
\SetAlgoHangIndent{5.5em}
%\SetAlgoNoLine
%\setlength{\algomargin}{0pt}
%\begin{enumerate}[ itemsep=-10pt, topsep=2pt]
%\item 
    \phantom{.}\text{\bf{Input:}} $U$ and $C$\\
    \phantom{.}\text{\bf{Output:}} \ $K_c$ and $C$, $\forall \ c \in C $ \\
\phantom{....} \nl \text{\bf{Initialize}} \ \textit{cluster head set  $C_\mathcal{CH} = \emptyset$ and $c=1$}; \\ 

\vspace{-9 pt} \hspace{-6 pt}\nl  \Indp\While{c \ \leq \ C}{    
\phantom{....} \nl    \it{\hspace{-16 pt}Randomly select a cluster head $\mathcal{CH}_c$ from $U$;} \\
\phantom{....} \nl      \it{\hspace{-16 pt}Update $C_\mathcal{CH} =\{\mathcal{CH}_c, \forall \ c \in C$\};}\\
\phantom{....} \nl         \hspace{-16 pt}c = c + 1;\\\vspace{-7 pt}}
\phantom{....-}\nl     \hspace{-18 pt} \Repeat{ \hspace{+4 pt}\it{The cluster members do not change}}
{ 
\phantom{...-} \nl         \it{\multiline{\hspace{-16 pt}For each user $m \in U$, calculate the minimum Euclidean distance \\\hspace{-16 pt}from the $\mathcal{CH}_c$;}}\\
\phantom{....} \nl         \it{\hspace{-16 pt}Fit each user to the closest cluster;}\\
\phantom{...-} \nl         \it{\multiline{\hspace{-16 pt}Update  the cluster head $\mathcal{CH}_c$ by taking the average of all \\\hspace{-16 pt}the users $m$; }}}
%\nl         \bf{until} \it{The cluster members do not change}\\
\caption{\small K-means user clustering in MU-MISO environment.}
\label{Algorithm1}
\end{algorithm}
  \end{spacing}
% \end{adjustwidth}
\end{minipage}

\begin{figure}[ht]
%\vspace{-24 pt}
	   \centering
	   \includegraphics[width=0.45\textwidth]{figures/UAVC/Clustering2.eps}
	    %\vspace{-9 pt}
        \caption{Channel-based clustering. %\hl{optional, can go if we do not have space} %\hl{Vuk: Would it make sense to also provide the other two clustering results (Fig. 4a, b, c) and label the UEs in the plot, e.g. from 1 to 16, so we can get an idea how their cluster association changes depending on the metric used? For now, let's keep just this example and relocate it}
        }
        %\vspace{-3 mm}
        \label{fig:Clustering}
\end{figure}

Algorithm 1 works with any metric contained in the data. One possible metric is the normalized channel,
\vspace{-5pt}
\begin{equation}
        h^n_{sk} = \frac{ h_{sk}}{\parallel h_{sk} \parallel_2},
    \label{eq:sim}
\vspace{-4pt}
\end{equation}
%$h^n$ is chosen 
which captures the variations of channel gains resulting from different RF propagation effects, such as small-scale fading and shadow fading.  Parameter $h_{sk}$ is the channel gain between the GBS and user $k$ and $\parallel.\parallel_2$ is the $L_2$ vector norm.  The similarity of channels between UEs and GBS is used to create two clusters and the cluster with a smaller number of UEs is chosen to be served by the UAV. This is because the larger cluster may require more movements from the UAV to support UEs in the larger cluster and that it consumes more power. Note that the UEs are not necessarily located close together or at the same spot. Figure~\ref{fig:Clustering} shows an example clustering outcome based on the normalized channel metric and Algorithm 1. It shows two clusters %, each with its centroid, 
which happen to have the same number of associated members. %%Note that the number or associated UEs per cluster is not necessarily balanced. %solution where the metric is the \hl{complex channel gain}. 

\textcolor{black}{%K-means clustering 
%Algorithm 1 can apply other similarity metric. 
Other metrics can be employed for this problem, such as distance based clustering or rate based clustering, where UEs with the nearest distance to the GBS and the highest downlink rates, respectively, would be grouped. % into one cluster. %, and channel base clustering. %, and eavesdropper rate base clustering. 
The metric can have an effect on the system performance and should be chosen based on the objective and the ability or simplicity to obtain the necessary information to calculate the value for each UE. %%, which may require feedback from the UE %, eavesdropper, 
%%or other nodes in the network.  %Other options include distance or \hl{rate based} clustering with respect to the GBS, for instance. 
}



==> include/proposed_sol_old.tex <==

The UAV chooses its trajectory and power level through a transition process based on current system state.
% 7The UAV’s trajectory and power consumption are based on the state transition process in which the UAV chooses its location and the UE’s power according to the current system state. 
Since the next state of the system is independent from the previous state and action, the process can be modeled as an MDP. This allows us to apply a reinforcement learning algorithm to an UAV agent without knowing the system model, and thereby achieving the optimal secrecy rates in the network. 
\textcolor{red}{Justify here or earlier why RL and why you consider Q-learning to solve this problem. Add citations to related works or the properties of Q/RL.}

In what follows, we first describe the MDP model by defining settings that includes states, actions, and the reward for the UAV agent. Then, we introduce the Q-learning method based on the defined MDP setting to solve the problem. Aiming to avoid the curse of dimensionality for high state-action space, we finally propose a deep Q-learning method in which a deep neural network is employed to estimate the action-value function for the UAV agent in the environment.

\subsection{MDP Settings}
The MDP for the UAV agent is composed of a state space $\mathcal{S}$, an action space $\mathcal{A}$, a reward space $\mathcal{R}$, and the transition probability space $\mathcal{T}$, i.e., $\mathcal{(S, A, R, T)}$. At time slot $t$, the agent observes the state $s_t \in \mathcal{S}$, and based on its policy, it  takes an action $a_t \in \mathcal{A}$. Depending upon the distribution of transition probability $\mathcal{T}(s_{t+1}|s_t, a_t)$, the agent will be transferred to the new state $s_{t+1}$. Since the transition probability is too dependent on a specific environment and it is difficult to obtain, we choose Q-learning method as a model-free algorithm to directly find the best policy for each action of each state. This means that we do not need to know $\mathcal{T}$, but we need to carefully define states, actions, and the reward of the agent as follows:

%\begin{itemize} [leftmargin=*]
\textbf{State:} The set of states is defined as 
\begin{equation}
\mathcal{S} = \{s_1, s_2, ..., s_t, .., s_T\},
\label{equ:MDP_state_set}
\end{equation}
where $T$ is the total time slots. Each state $s_t$ at a time slot $t$ has three elements that are defined as follows:
\begin{equation}
s_t =\{\Delta x, \Delta y, \Delta z \}, 
\label{equ:MDP_states}
\end{equation}
where $\Delta x, \Delta y$, and $\Delta z$ represent the distance between the UAV and each UE on $x, y$, and $z$ axes, respectively. For example, $ \Delta y = y_u - y_i$.  It is worth nothing that the value of each state directly affects the channel gain, hence SNR.

\textbf{Action:} The states are transited according to the defined actions of the UAV. A set of actions is defined as
\begin{equation}
\mathcal{A} = \{a_1, a_2, ..., a_t, .., a_T\},
\label{equ:MDP_actn_set}
\end{equation}
where each action for the UAV at time $t$, i.e., $a_t$, consists of two parts of movements and one part of power changes, That is 
\begin{equation}
a_t = \{\delta_x, \delta_y, \delta_p\},
\label{equ:MDP_Actions}
\end{equation}
where $\delta_x$ and $\delta_y$ represent the movements in $x$ direction and $y$ direction, respectively. Also, $\delta_p$ denotes the change of power. For the sake of simplicity and without loss of generality, the altitude of the UAV is assumed to be constant (i.e., $\delta_z = cte$).

As a sample configuration, the movements, i.e., $\delta_x$ and $\delta_y$, can be assumed to change by $+1$ unit or $-1$ unit, and the power level, i.e., $\delta_p$, can be assumed to change by $p_1$, $0$, or $-p_1$, where $p_1$ is an arbitrary number. Hence, here, we consider $4$ possible directional movements and $3$ power level changes, resulting in $12$ possible actions for the UAV in one state of the environment. For example, one action of the UAV agent at time slot $t$ could be $ a_t = \{x+1 , y-1, P + p_1\}$, which implies that the UAV increases its $x$ direction by $1$ unit, decreases its $y$ direction by $1$ unit, and increases its power by $p_1$.

%For the sake of simplicity and without loss of generality, the altitude of the UAV is assumed to be constant (i.e., $\delta_z = cte$), and the movement of the UAV is assumed to be in the $x$ and $y$ axes. The moving along $x$ and $y$ directions can take one of $+1$ or $-1$ values, and the power level changes can take on of the three following values $\{+p_1, 0, -p_1\}$, where $p_1$ is an arbitrary number.

 \textbf{Reward:} After taking an action $a_t$ in a state $s_t$ at time slot $t$, the UAV agent will receive a reward $R_t(s_t, a_t)$. We define the reward function of the system based on the instantaneous secrecy rate as follows:
\begin{equation}
    {R_t(s_t, a_t)} = \bigg(
    C_{u}[t]- C_{j}[t] \bigg)^+.
    \label{equ:totalsec}
\end{equation} 
Therefore, the UAV will get more rewards for the actions that leads it to the higher secrecy rates.

%\textcolor{red}{Can we have a small example illustration related to the problem that shows the states, actions, rewards, and Q-Table? Some people provide a toy problem to illustrate the problem at the beginning of the paper. Here we can make it focused on our problem.}

\subsection{Q-learning Method}
The UAV agent can apply the Q-learning method in order to find the best policy for the state-action relationship. Q-learning is a classical table-based reinforcement learning algorithm in which the state-action pair has the value of $Q(s,a)$. The rows of the Q-table consist of the states of the environment and the columns of the Q-table represent the possible actions of the UAV agent. For example, for the aforementioned sample of states and actions, the table has $3$ rows and $12$ columns. The Q-values in the table are initially filled by random numbers. Then, each state-action pair of the table is updated according to the following equation \textcolor{red}{Where does this eq. come from, or is it your contribution? Explain this and provide more context, if possible, why you chose it and why it is suitable. If it comes directly from [13], cite it right before the colon}:
\begin{flalign}
\notag  Q^{\text{new}}(s, a) = & \ (1-\alpha) \ Q(s, a) \ + \ \alpha \ \times \\
 &  E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
 \label{eq:Bellman}
 \end{flalign}
where the $s^\prime$ and $a^\prime$ are the next state and action, respectively. Also, the parameter $\gamma \in (0,1)$ denotes the discount factor that affects the importance of the future reward. In particular, when the $\gamma$ goes to $0$ (or $1$), the UAV agent puts more weight on the immediate (or future) reward. The parameter $\alpha$ refers to the learning rate which indicates how quickly an agent leaves the previous Q-value for the new Q-value in the table. The second term of (\ref{eq:Bellman}) is called Bellman equation. In each step, the Q-value is updated while applying the $\epsilon-$greedy algorithm. This algorithm provides a balance between the exploration and the exploitation of the UAV agent in the environment \cite{Survey17deep}.


Although the Q-learning provides a general framework for reinforcement learning, it requires to store the Q-values for each state-action pair in the table. The number of state-action pairs in the table quickly increases with the number of UEs, UAV directions, and power levels. As the Q-table becomes larger and larger, the storing and the updating process of the table becomes more time-consuming and can become impractical. This leads us to consider the Deep Q-network RL method where a deep neural network is used to estimate the $Q(s, a)$ values in the environment, as opposed to Q-learning where Q-table is used to estimate the state-action values. This has advantages in terms of handling the large number of states and actions and decreasing the processing time.

%\hl{.... This has advantages in terms of efficiency and flexibility Fig.}~\ref{fig:DQL} \hl{illustrates our design.}


%based on the well-known Bellman equation:
% \begin{equation}
%     Q(s, a) = E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%     \label{eq:Bellman}
% \end{equation}

% In each iteration, the value of $Q(s, a)$ is updated by the following equation:
% \begin{equation}
%     Q^{\text{new}}(s, a) = (1-\alpha) \ Q(s, a) \ + \ \alpha \\
%     E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%     \label{eq:Bellman}
% \end{equation}


\begin{figure}[t]
  \centering
  \includegraphics[width=8.5cm,height=6.5cm]{figures/Fig_AB_DQL.pdf}
  \caption{Block diagram of the DQN-based UAV optimal secrecy rate system.}
  \label{fig:DQL}
\end{figure}


\subsection{Deep Q-learning Method}
Deep Q-network (DQN) learning algorithm, initially proposed by Google Deep Mind \cite{DeepMind2015}, integrates the reinforcement learning and deep learning methods. This technique uses the power of nonlinear functions, such as deep neural networks (DNNs), in order to approximate Q-values and handle high dimensional state-action problems. In this section, we propose a DQN-based algorithm in order to maximize the secrecy rate between the UAV and the UE in presence of an eavesdropper in the environment.

Fig. \ref{fig:DQL} shows the block diagram of the proposed DQN-based method. %As can be seen, there exits 
There are two DNNs of the same structure: a training network and a target network. The training network outputs the Q-values associated with the actions of the UAV in each state. The target network, however, supervises the training network by providing the target Q-values obtained from the Bellman question. The target values are compared with the outputs of the training network in order to minimize the loss function described below. Also, the target network prevents the learning model from suffering from the noise in the environment. The inputs to the networks are the states of the UAV agent in the environment, see (\ref{equ:MDP_state_set})-(\ref{equ:MDP_states}). 
The outputs of the network are the Q-values corresponding to the actions of the UAV agent, i.e., $Q(s, a; \theta)$, where $\theta$ denotes the weights of the DNNs.

As the UAV takes an action in the environment, the system generates a record of experience. At time step $t$, the experience contains the current state $s_t$, the action $a_t$, the reward $r_t$, and the next state $s_{t+1}$, formed as a tuple $e_t = (s_t, a_t, r_t, s_{t+1})$. Each such experience is stored in a replay memory with the capacity of $N$, such that $\mathcal{M}=\{e_1, ..., e_t, ..., e_N \}$. The memory is a queue-like buffer that stores the latest N experience vectors. 
We use a min-batch sample from the replay memory in order to feed the input of the training network as shown in Fig.~\ref{fig:DQL}. The main reason for using the mini-batch samples from the reply memory is to break possible correlations between sequential states of the environment, and thereby facilitate \hl{better} learning.

In order to minimize the error prediction of the DNNs, a loss function is used that is defined as %follows:
\begin{flalign}
\notag L(\theta) = \mathbb{E} \Bigg[ \bigg( \Big[ r_t + \gamma \times \max_{a\in \mathcal{A}} \ Q(s_{t+1}, a_{t+1}; \theta^{\dagger})\Big] - \\ 
\Big[Q(s_{t}, a_{t}; \theta) \Big] \bigg)^2 \Bigg],
\label{eq:loss}
\end{flalign}
where the Q-value of the first term is obtained from the target network and the Q-value of the second term is obtained from the training network. In the equation, the parameters $\theta^{\dagger}$ and $\theta$ denote the coefficients of the target network and training network, respectively. The $\theta^{\dagger}$ coefficients are updated every few time slots in order to ensure the stability of the target values and, hence, facilitate stable learning. 

The UAV applies a gradient descent algorithm,
\begin{flalign}
\notag \nabla_{\theta}\, L(\theta) &= - \mathbb{E} \Bigg[ 2 \ \nabla_{\theta}Q(s_{t}, a_{t}; \theta) \bigg( \, r_t + \, \gamma \ \times \\ & \qquad \max_{a\in \mathcal{A}} \ Q(s_{t+1}, a_{t+1}; \theta^{\dagger})  - Q(s_{t}, a_{t}; \theta) \bigg)  \Bigg],
\label{eq:GDS}
\end{flalign}
to update the $\theta$ \hl{and} $\theta^{\dagger}$ \hl{parameters} of the DNNs with the aim of minimizing the prediction error.

Finally, we apply the $\epsilon-$greedy algorithm to select an action while balancing the exploration and the exploitation of the UAV in the environment (Fig.~\ref{fig:DQL}). In this algorithm, the UAV explores the environment with the probability of $\epsilon$ by choosing a random action (i.e., movement and power level). The UAV, however, exploits the environment with the probability of $1-\epsilon$ by choosing the actions that maximizes the Q-value function, i.e., $a^{*} = \text{argmax}_{a \in \mathcal{A}} \ Q(s,a; \theta)$. A high value of $\epsilon$ is initially set in the model for the UAV to spend more time for the exploration. As the agent obtains more knowledge about the environment, the $\epsilon$ value is gradually decreased to leverage the experiences and choose the best actions by the UAV, rather than continuing the exploration. The detail of the DQN-based algorithm used by the UAV agent for optimizing secrecy rates is presented in Algorithm 1. \textcolor{red}{What is the method that you used to come up with this algorithms. Explain the optimization, initial parameter section, and dependency on parameters and walk us through Algorithm 1 (with line numbers). Are you directly maximizing the secrecy rate, i.e. Fig. 2 know the eavesdropping rate? Where will Fig. 2 be implemented in a real network (at the UAV)?}


















% ----------------------
% ----------------------
% ----------------------
% ----------------------
% AB's Algorithm!
% ----------------------

 \begin{minipage}{0.95\linewidth}
%  \begin{adjustwidth}{1em}{}
\begin{algorithm}[H]
\footnotesize
\SetAlgoLined
%\begin{enumerate}[ itemsep=-10pt, topsep=2pt]
%\item 

\text{\bf{Initialize}} \epsilon_{start}, \epsilon_{end}, decay\\
\text{\bf{Initialize}} \ \textit{T, N}, \textit{K} \ (Total \ epochs)   \\
\text{\bf{Initialize}} \ \theta, \theta^{\dagger}, \gamma, \alpha, \textit{B} %\ (Target \ network \ update \ cycle) \\ 

\For{episode = 1, 2, ..., K}
{    
    \it{Reset Environment} \\
    \For{t = 1, 2, ..., T}
    {
        s_t = (\Delta x_t, \Delta y_t, \Delta z_t)\\
        Select \ action \ using \  \epsilon-greedy:
        
        \bf{if} \ \epsilon>random(0,1) \ \bf{then} \\
        |\qquad    \it{Select \ random \ a_t \in \mathcal{A}}\\
        \bf{else}\\
        |\qquad    \it{a_t = \argmax_{a \in \mathcal{A}} \  Q(s_t,a; \theta) }\\
        \bf{end}\\
        \it{UAV \ takes \ an \ action, \ a_t}\\
        Obtain \ s_{t+1}, \ r_{t} \\
        Replay \ Memory: \mathcal{M} \gets  \mathcal{M} \ \cup \{s_t, a_t, r_t, s_{t+1} \}\\
        Minibatch\ from \ \mathcal{M}: e_i=(s_i, a_i, r_i, s_{i+1})\\
        Train \ the \ DNN \ training \ network \\
        Update \ \theta  \ in \ training \ network \ via \ eq. \ (\ref{eq:GDS})\\
        Update \ \theta^{\dagger} \ in \ target \ network \ every \ B \ steps

    }
    $\epsilon \gets$ update $ \epsilon$ \\
    Store secrecy rate for each epoch




%   
  
 }
 \KwResult{Optimal Secrecy Rate in eq. (\ref{eq:opt_secrecy_rate})}
    %\textbf{until} $\Vert \nabla_{R} \xi(\vartheta) \Vert_2 \leq \chi$\\
\caption{\small DQN-based UAV for optimizing secrecy rate.}
\label{Algorithm1}
\end{algorithm}
% \end{adjustwidth}
\end{minipage}
  

%   \begin{minipage}{0.95\linewidth}
% %  \begin{adjustwidth}{1em}{}
% \begin{algorithm}[H]
% \footnotesize
% \SetAlgoLined
% %\begin{enumerate}[ itemsep=-10pt, topsep=2pt]
%     %\item 

%     Initialize $P^{(0)}$, $x_u^{(0)}$, $y_u^{(0)}$, and the initial slack variable $\psi^{(0)}$ to feasible values and set $j=0$;
%     %\item 
    
%     Calculate $C^{(0)}=f_{P2}(P^{(0)}, x_u^{(0)}, y_u^{(0)})$ according to~(\ref{13});
    
%     \While{ $\frac{C^{(j)}-C^{(j-1)}}{C^{(j)}} \leq \chi$}
%   {
%         With given $P^{(j-1)}$, set the new feasible points $x^{(j)}_{u(fea)}=x^{(j-1)}_u$, $y^{(j)}_{u(fea)}=y^{(j-1)}_u$, and $\psi^{(j)}_{(fea)}=\psi^{(j-1)}$;
        
%         Calculate the new trajectory update $(x^{(j)}_u,y^{(j)}_u)$ and the slack variable $\psi^{(j)}$  according to~(26);
        
%         Solve equation (19) with the obtained trajectory $(x^{(j)}_u,y^{(j)}_u)$ to calculate the updated transmission powers $P^{(j)}$;
        
%         Calculate the new $C^{(j)}=f_{P2}(P^{(j)}, x_u^{(j)}, y_u^{(j)})$ according to~(\ref{13});
   		
%   		$j \Leftarrow j+1 $
   		
%   }
%   \KwResult{Optimal $P$, $x_u$ and $y_u$ }
%     %\textbf{until} $\Vert \nabla_{R} \xi(\vartheta) \Vert_2 \leq \chi$\\
%  \caption{\small Proposed algorithm for optimizing the transmission power and UAV position.}
%  \label{Algorithm1}
% \end{algorithm}
% % \end{adjustwidth}
%   \end{minipage}



























%  \begin{figure}[t]
%      \centering
%      \includegraphics[width=16cm,height=10cm]{figures/Fig_AB_DQL.pdf}
%      \caption{The simulation scenario.}
%      \vspace{-5mm}
%      \label{fig:system}
%  \end{figure}
 

%  \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.8]{figures/Fig_AB_DQL.pdf}
%      \caption{DQL.}
%      \vspace{-5mm}
%      \label{fig:system}
%  \end{figure}




\color{black}
\color{black}

==> include/qlearning.tex <==
\subsubsection{Q-Learning Method}
%The UAV agent can apply the Q-learning method to find the best policy for the state-action relationship. 
Q-learning is a classical table-based RL algorithm in which a state-action pair has the value of $Q(s,a)$. The rows and columns of the Q-table thus consist of the environmental states and %the columns of the Q-table represent the 
possible actions of the, respectively. %For example, for the aforementioned sample of states and actions, the table has $3$ rows and $12$ columns.
The Q-values in the table are initially filled by random numbers. Then, the Bellman equation \cite{Survey17deep}, 
%by means of iterative updates \cite{Survey17deep}:
%each state-action pair of the table is updated according to the Bellman equation 
\begin{flalign}
Q^{*}(s, a) = E_{s^\prime}\bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\bigg],
 \label{eq:Bellman}
 \end{flalign}
% \textcolor{red}{Where does this eq. come from, or is it your contribution? Explain this and provide more context, if possible, why you chose it and why it is suitable. If it comes directly from [13], cite it right before the colon}:
% \begin{flalign}
% \notag  Q^{\text{new}}(s, a) = & \ (1-\alpha) \ Q(s, a) \ + \ \alpha \ \times \\
%  &  E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%  \label{eq:Bellman}
%  \end{flalign}
is used to obtain the optimal state-action pairs, where $s^\prime$ and $a^\prime$ symbolize the next state and action. Parameter $\gamma \in (0,1)$ denotes the discount factor that affects the importance of the future reward. %In particular, when the $\gamma$ goes to $0$ (or $1$), the UAV agent puts more weight on the immediate (or future) reward. 
%In order to update each state-action pair of the table, the following equation is used
% \begin{flalign}
% \notag  Q^{\text{new}}(s, a) = & \ (1-\alpha) \ Q(s, a) \ + \ \alpha \ \times \\
%  &  E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%  \label{eq:Bellman}
%  \end{flalign}
The Bellman equation is used through an iterative process to update the Q-values, where
%As part of the updating process for the Q-values, 
a learning rate parameter $\alpha$ is applied to determine how quickly an agent leaves the previous Q-value for the new Q-value in the table. That is, $Q^{\text{new}}(s, a) = (1-\alpha) \ Q_{i-1}(s, a) + \alpha \ Q_{i}(s, a)$, where subscript $i$ %indicates the $i$-th 
iteration. % in the process. 
Finally, %in each step,
the $\epsilon-$greedy algorithm is used to balance between exploration and exploitation of %the UAV agent in 
the environment for updating the Q-value %is updated while applying . This algorithm 
\cite{Survey17deep}.



%where the parameter $\alpha$ refers to the learning rate which indicates how quickly an agent leaves the previous Q-value for the new Q-value in the table. The second term of (\ref{eq:Bellman}) is called Bellman equation. 



Although Q-learning provides a general framework for RL, it requires to store the Q-values for each state-action pair in the table. The number of state-action pairs in the table grows quickly with the number of states and actions %. %UEs, UAV directions, and power levels. 
%As the Q-table becomes large%larger and larger
%, the %storing and the updating 
%process %of the table 
and can become more time-consuming and %can become 
impractical. %This leads us to 
Therefore, we consider the DQN method where a DNN is used to estimate the $Q(s, a)$ values. %in the environment
%, as opposed to Q-learning, where the Q-table is used to estimate the state-action values. 
This has advantages in terms of handling a large number of states and actions and the associated processing time.
%\hl{.... This has advantages in terms of efficiency and flexibility Fig.}~\ref{fig:DQL} \hl{illustrates our design.}
%based on the well-known Bellman equation:
% \begin{equation}
%     Q(s, a) = E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%     \label{eq:Bellman}
% \end{equation}

% In each iteration, the value of $Q(s, a)$ is updated by the following equation:
% \begin{equation}
%     Q^{\text{new}}(s, a) = (1-\alpha) \ Q(s, a) \ + \ \alpha \\
%     E\Bigg[R(s, a) + \gamma \times \max_{a\in \mathcal{A}} \ Q(s^\prime, a^\prime)\Bigg],
%     \label{eq:Bellman}
% \end{equation}


==> include/related.tex <==
\textcolor{red}{It is good practice to have a separate section. Where space is limited, it can be included in the intro or other parts. Also we need to compare our results and conclusions to those from recent related works, those that apply, later in the paper.}

==> include/simulation_parameters_table.tex <==

\begin{table}[t]
%\fontsize{12}{10}\selectfont
%\fontsize{6}{10}\selectfont
\centering
\caption{Simulation parameters.}
\label{tab:parameters}
\resizebox{0.35\textwidth}{!}
{%
\begin{tabular}{|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Parameter}\end{tabular}     & \textbf{Value}                              \\ \hline
%\begin{tabular}[c]{@{}c@{}} $\textit{L}_\textit{x}$\end{tabular} & 10 m  \\ \hline
%\begin{tabular}[c]{@{}c@{}} $\textit{L}_\textit{y}$\end{tabular} & 10 m   \\ \hline
%\begin{tabular}[c]{@{}c@{}} Urban environment constants A and B\end{tabular} & A=11.95, B=0.136 \\ \hline
%\begin{tabular}[c]{@{}c@{}} The height limits of AIAB ($\text{h}_\text{min},\text{h}_\text{max}$)\end{tabular} &  (50,100) \\ \hline
\begin{tabular}[c]{@{}c@{}}Area length ($L_x$) \end{tabular} & %\hl{$L_x$ = 
20 m\\\hline
\begin{tabular}[c]{@{}c@{}}Area width ($L_y$)\end{tabular} & %$L_y$ = 
20 m\\\hline
\begin{tabular}[c]{@{}c@{}}  UAV height ($z_u$) %limits of AIAB
\end{tabular} & %$h_{min}$=35, $h_{max}$=100 m
%$z_u$ = 
20-%$	\sim$
80 m\\ \hline
\begin{tabular}[c]{@{}c@{}}  {UAV trajectory step along the \textit{x} or \textit{y} axis}  %limits of AIAB
\end{tabular} & %$h_{min}$=35, $h_{max}$=100 m
%${\delta x, \delta y, \delta z}$ = 
0.5 m\\ \hline
\begin{tabular}[c]{@{}c@{}}  {UAV trajectory step along the \textit{z} axis}  %limits of AIAB
\end{tabular} & %$h_{min}$=35, $h_{max}$=100 m
%${\delta x, \delta y, \delta z}$ = 
2 m\\ \hline
\begin{tabular}[c]{@{}c@{}} GBS height ($z_s$)\end{tabular} & %$z_s$=
15 m\\\hline
\begin{tabular}[c]{@{}c@{}}Path loss at 1 m reference distance ($\lambda_0$) \end{tabular} & %$\lambda_0 =$$%7 \times 10^{-5}
-40 dB \text{~\cite{sky}}             \\ \hline
% \begin{tabular}[c]{@{}c@{}} Environment constants\end{tabular} &  A=11.95, B=0.136  \\ \hline
% \begin{tabular}[c]{@{}c@{}} LoS Path loss parameters\end{tabular} & $\chi_{_{LoS}}$=10.34, $\delta_{LoS}$=2.42 \\ \hline
% \begin{tabular}[c]{@{}c@{}} NLoS Path loss parameters\end{tabular} & $\chi_{_{NLoS}}$=13.11, $\delta_{NLoS}$=4.28 \\ \hline
% \begin{tabular}[c]{@{}c@{}} The ABG channel parameters\end{tabular} & $\rho_{G}$=2.1, $\beta$=31.7, $\gamma_{G}$=2 \\ \hline
% \begin{tabular}[c]{@{}c@{}} The shadowing standard deviation \end{tabular} & $\sigma_{sh}$=3.9 \\ \hline
\begin{tabular}[c]{@{}c@{}}  Path loss exponent ($\alpha$) \end{tabular} & %$\alpha=$ 
2 \\ \hline
\begin{tabular}[c]{@{}c@{}}  Rician factor ($\beta$)\end{tabular} & %$\beta =$ 
10 dB \\ \hline
\begin{tabular}[c]{@{}c@{}} \textcolor{black}{ABG distance-dependent exponents} (\rho_{G})\end{tabular} & \textcolor{black}{2.1} \\ \hline
\begin{tabular}[c]{@{}c@{}} \textcolor{black}{ABG intercept} (\jmath)\end{tabular} & \textcolor{black}{31.7 dB} \\ \hline
\begin{tabular}[c]{@{}c@{}} \textcolor{black}{ABG frequency-dependent exponents} (\gamma_{G})\end{tabular} & \textcolor{black}{2} \\ \hline 
\begin{tabular}[c]{@{}c@{}} \textcolor{black}{Shadow fading} (\chi_{\sigma}^{G2G})\end{tabular} & \textcolor{black}{3.9 dB} \\ \hline
\begin{tabular}[c]{@{}c@{}} Central frequency\end{tabular} & 3.2 GHz \\ \hline
\begin{tabular}[c]{@{}c@{}} Noise variance\end{tabular} & 10$^{-2}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of ground users (K)\end{tabular} & %K = 
4-%$\sim$
64 \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of ground eavesdroppers (E)\end{tabular} & %E = 
2-%$\sim$
10 \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of K-means clusters (R) \end{tabular} & %R = 
2 \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of episodes\end{tabular} & 2 $\times$ 10$^{4}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Number time slots per episode\end{tabular} &  200 \\ \hline
\begin{tabular}[c]{@{}c@{}} Learning rate (LR)\end{tabular} & % LR = 
10$^{-4}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Discount factor\end{tabular} & 0.9 \\ \hline
%Noise variance                                                     & 10^{\text{-12} }       \\ \hline
%\begin{tabular}[c]{@{}c@{}}
%SNR at the reference point\end{tabular}                                                      & 90 dB       \\ \hline
%\begin{tabular}[c]{@{}c@{}}dx    \end{tabular}        & 20 m                               \\ \hline
%M                                                          & 5 users                              \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of DNN layers\end{tabular} & 4 \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of NN nodes\end{tabular} &  \\ \hline
\begin{tabular}[c]{@{}c@{}} Replay memory size\end{tabular} & 10$^{5}$ entries \\ \hline
\begin{tabular}[c]{@{}c@{}} Mini-batch size\end{tabular} & 64 \\ \hline
\begin{tabular}[c]{@{}c@{}} Update rate of target network\end{tabular} & 10 \\ \hline
% \begin{tabular}[c]{@{}c@{}} Batch size\end{tabular} & 50 \\ \hline
% \begin{tabular}[c]{@{}c@{}} Update rate of target network\end{tabular} & 10 \\ \hline
% Bandwidth                                                          & 10 MHz                              \\ \hline
\end{tabular}%
}
%\vspace{-5mm}
\end{table}

==> include/system_Unrelated.tex <==
 \begin{figure}[t]
     \centering
     \includegraphics[width=0.40\textwidth]{figures/SystemModel_DQLUAV.eps}
     \caption{The simulation scenario.}
     \vspace{-5mm}
         \label{fig:system}
 \end{figure}
 We consider a HetNet deployment as shown in Figure 1, macro cells base station (MBS) is deployed with uniform planar array (UPA) to provide mmWave backhaul links for aerial base stations (ABS). In addition, ABS is also deployed with UPA to offer a higher reliable access and mmWave data transmission for UEs that are located in blind coverage where the connection between MBS and user equipment (UE) is suspended due to blocking, interfering or too far away. UEs are distributed randomly in the involved area. we define the achievable rates of both access $C_A$, and backhaul $C_B$ links for the ABS as 
\begin{equation}
    {C _{A}} = \log_2 (1+\gamma_A),
\end{equation}
\begin{equation}
    {C _{B}} = \log_2 (1+\gamma_B),
\end{equation}
where 
\begin{equation}
    \begin{aligned}
    {\gamma _{A}} %&= \frac{Y_A}{\sigma^2 + I_{A}},\\
    %&
    = %\frac{P_a H^{LoS}_a}{\sigma^2 + \sum\limits_{i\in K}P_a H^{LoS}_{i,a}}
    \frac{P_a G_a}{\sigma^2} 
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}
    {\gamma _{B}} %&= \frac{Y_A}{\sigma^2 + I_{A}},\\
    %&
    = %\frac{P_B H^{LoS}_a}{\sigma^2 + \sum\limits_{i\in K}P_a H^{LoS}_{i,a}}
    \frac{P_B G_B}{\sigma^2} 
    \end{aligned}
\end{equation}
where $P_A$ and $P_B$ denote the transmit power for the access and backhaul links, respectively. While, the $G_A$ and $G_B$ define the channel gain of the access and backhaul link, respectively. The $H$ can be further defined as follow
\begin{equation}
        H =  PL(d)+H_{BF}+\Upsilon(\eta^2)   
\end{equation}
where PL is the path loss component, which is defined in mmWave LoS transmission as $PL=61.4+20log_{10}(d)$, $d$ is the distance between transmitter and receiver, $H_BF$ is the directional beamforming antenna gain, $\Upsilon(\eta^2)$ is the log-normal shadowing in dB, which is a zero-mean Gaussian random variable with variance $\eta^2$. Therefore, the rate of the ABS under the integrated access and backhaul links is given as follow
\begin{equation}
        C =  min\{C_A, C_B\}
\end{equation}
% The scenario of interest that we considered for this paper is illustrated in~Fig.~\ref{fig:system}. The ground user communicates with ABS provided by the aerial node in the presence of terrestrial eavesdropper.  
% The ground user and eavesdropper are randomly distributed within a predefined grid dimension. 
% The ABS is positioned to provide a secure and reliable uplink (UL) communication traffic for the user under attack via the 3D mobility and strong LoS communications over the terrestrial communication links supplied by the terrestrial base stations. 
% Without loss of generality, in this paper we model and analyze the UL channel. The same principles can be applied for the DL.

% %The set of $M$ users in the cluster %being attacked 
% %and the set of $K$ eavesdroppers are denoted as $V=\{V_i|i=1,2,...,M\}$ and $E=\{{E}_{j}|j=1,2,...K\}$, respectively.
% %Without loss of generality, 
% We define the location of the ABS, the eavesdropper, and the user in the 3D Cartesian coordinate system as ($x_u,y_u,z_u$) , ($x_j,y_j,z_j$), and ($x,y,z$), respectively.
% %%The UAV flies at the % has a fixed 
% %%altitude $z_u$, which may be chosen according to %considered as
% %%the minimum height at which the UAV will have line of sight (LoS) links with the users in the cluster%, and where it would avoid buildings and obstacles from the air
% %%~\cite{UAVLoS}. 
% %%The UAV relay operation %along the cluster travel distance
% %%will be executed over a finite duration $T$. 
% For practicality, %we distribute the UAV relaying period over $N$ 
% time slots are used to capture the different radio frames and statistical channel conditions, as well as the momentarily static position of the ABS, users, and eavesdroppers. %, equally. 
% Therefore, the ABS coordinates in time slot $t$ will be expressed as ($x_u[t], y_u[t], z_u[t]$).    


% \subsection{Communications Channel} The received signal at the ABS when the ground UE initiate the transmission process for sending the signal $s$ with power $P$ is given as
% %\vspace{-1 mm}
% \begin{equation}
%     {r} = \sqrt{P\hbar}s+n,
%  %  \vspace{-2 mm}
% \end{equation}
% where $\hbar$ is corresponding to the air-to-ground (A2G) channel power gain between the ground UE and the ABS, and $n$ denotes the additive white Gaussian noise (AWGN) of zero mean and $\sigma^2$ variance. %
% Based on the measurements presented in~~\cite{sky}, we can assume that the LoS channel model is a good approximate to model the A2G channel in rural areas specifically when the UAV flies at higher altitudes.% 80 m.  
% The channel gain %${g}_{iu}[n]$ 
% %in time slot $n$ 
% has %is characterized by
% a path loss exponent of two and can be written as
% %\vspace{-1 mm}
% \begin{equation}
% \small
% \begin{aligned}
%     \hbar[t] &=\zeta_{0}d^{-2}_{u}[t] \\
%     &=\frac{\zeta_0}{(x[t]-x_u[t])^2+(y[t]-y_u[t])^2+(z[t]-z_u[t])},
%     \end{aligned}
%     \label{eq:channel_gain1}
% \end{equation}
% where $\zeta_{0}$ is the channel gain at the reference point of $d_0$ = 1 m. The $\zeta_{0}$ for the A2G channel model and ground-to-ground (G2G) will not be differentiate     due to use the same the antenna gains and the carrier frequency for both cases. Parameter $d_{u}[t]$ denotes the distance between the ground user and the ABS. 

% The capacity of the channel between the ground UE and the ABS in time slot $t$ is calculated as follows: 
% %\vspace{-1 mm}
% \begin{equation}
% %\small
% %\begin{aligned}
%     {C _{u}[t]} = \log_2 \left( 1+\frac{{P}[t]\hbar[t]}{\sigma^2}\right) = \log_2 \left( 1+\frac{\zeta_0{P}[t]}{d^2_{u}[t]\sigma^2}\right),
%     %{(x_i[n]-x_u[n])^2+(y_i[n]-y_u[n])^2[n]+(z_i[n]-H)^2}
% %\end{aligned}
% \end{equation}
% where $\zeta_0/\sigma^2$ is the signal-to-noise ratio (SNR) at the reference point. 

% \subsection{Eavesdropping Channel} %{Because the UAV is in the air and can often establish an LoS link with the BS, beamforming and PC can be effectively employed to focus the radio frequency (RF) transmission between the BS and UAV. %and reduce the radiated energy. 
% The restricted space and size of the ground users such as the small Internet of things (IoT) devices and sensors, smartphones and portable devices enforce the use of single or fewer transmit antenna per each user, which is commonly transmit in broadcast mode without beamforming or directed behavior. Therefore, the UL links will not be focused and can be easily comprised. %Assuming ground eavesdroppers, here we therefore consider the user-UAV link being the dominant eavesdropping channel.

% The eavesdropper is going to wiretap the transmitted signal from the ground user, which can be formulated as follow
% %\vspace{-2 mm}
% \begin{equation}
%     {v } = \sqrt{P{\emptyset}}s+w,
% %    \vspace{-2 mm}
% \end{equation}
% where $w$ denotes the zero-mean 
% AWGN with a variance of $\sigma^2$ 
% at the eavesdropper. 
% As a result of the G2G communication link between the UE and the eavesdroppers, the exponent of the path loss for this link is assumed to be four. Within the time slot $t$, the G2G channel power gain represented by $\emptyset$ between the UE and eavesdropper can be modeled as
% \vspace{-0.5 mm}
% \begin{equation}
% \small
% \begin{aligned}
%     %{w}_{ij}[n] &=\omega_{0}d^{-4}_{ij}[n]\\
%     %=&\frac{\omega_0}{({(x_i[n]-x_j[n])^2+(y_i[n]-y_j[n])^2+(z_i[n]-z_j[n])^2)}^2},
%     \emptyset &=\zeta_{0}d^{-4}_{j}[t]\\
%     =&\frac{\zeta_0}{({(x[t]-x_j[t])^2+(y[t]-y_j[t])^2+(z[t]-z_j[t])^2)}^2},
%     \end{aligned}
% \end{equation}
% where $d_{j}[t]$ is the distance between the transmitter UE and the eavesdropper in the $t$th time slot.
% The corresponding capacity of the wiretap channel is 
% %\vspace{-2 mm}
% \begin{equation}
% %\small
% %\begin{aligned}
%     {C _{j}[t]} = \log_2 \left( 1+\frac{{P}[t]{\emptyset}[t]}{\sigma^2}\right) = \log_2 \left(
%     1+\frac{\zeta_{0}{P}[t]}{d^{4}_{j}[t]\sigma^2}\right).
%     %1+\frac{\delta_0{P_i}[n]}{d^{4}_{ij}[n]})\right),
%     %(x_i[n]-x_j[n])^2+(y_i[n]-y_j[n])^2[n]+(z_i[n]-z_j[n])^2
%  %   \end{aligned}
% \end{equation}

% %where $\delta_0=\omega__0/\sigma^2$ is the signal-to-noise ratio(SNR) at the reference point. 

% %This work considers the case of uncoordinated eavesdropping attacks. 
% %between the available eavesdroppers. 
% %%Therefore, if the transmission between the BS and $V_i$ has been interpreted successfully by any eavesdropper, the transmission will be exposed to other attackers. 
% %As a result of that, 
% %\textcolor{blue}{ We assume that the UE-AR links are subject to eavesdropping, whereas the BS-AR link can be more focused and is therefore less susceptible to eavesdropping.}


% % As a result, the capacity of the eavesdropping channel is calculated as the maximum %achieved 
% % capacity among the $K$ eavesdroppers:
% % \vspace{-2.5 mm}
% % \begin{equation}
% %     {C _{ij}[n]} = \max\limits_{j \in E} C _{ij}[n] = \max\limits_{j \in E} \log_2
% %     \left( 1+\frac{\lambda_0{P_i}[n]}{d^{4}_{ij}[n]}\right).
% %     %\left( 1+\frac{\delta_0{P_i}[n]}{d^{4}_{ij}[n]}\right),
% % \end{equation}
% % \vspace{-10mm}
% \subsection{Secrecy Capacity Metric}
% The security of the system is evaluated using the secrecy capacity metric which is a common metric that has been employed in the literature for analyzing various eavesdropping security problems in wireless communication networks.   
% The secrecy capacity is the positive divergence level that occurs when the legitimate channel capacity increases over the wiretap channel capacity, and the rate at which malicious node cannot decode any further data~\cite{YanWanGer2015}. %  which is associate to the rate at which no data will be decoded by the eavesdropper~\cite{YanWanGer2015}.  
% The average secrecy capacity over $T$ radio time slots with a scenario consisting of a ground eavesdropper, UE, and ABS is then obtained as
% %\vspace{-2 mm}
% \begin{equation}
%     {C_{sec}} = \frac{1}{T}\sum\limits_{t=1}^T \bigg(
%     C_{u}[t]- C_{j}[t] \bigg)^+,
%     \label{equ:totalsec}
% \end{equation}
% %\vspace{4 mm}
% where $[\omega]^+$ returns the maximum value between the provided $\omega$ and the null value.

% \subsection{Problem Formulation}
% The objective of this paper is maximizing the legitimate capacity $C_{u}$  
% by selecting the optimal position for the ABS and  
% performing optimal transmission power policy. 

% The optimization of the UE capacity will resultant an enhancement of the secrecy capacity under passive eavesdropping. %is relying on enhancing the UL capacity of the legitimate UE.
% However, the UL capacity of the ground user is dependent on having a short distance to the ABS  
% with strong LoS connections. % with the effected UEs. 
% Therefore, the ABS position constraint is formulated as follows:

% \begin{equation}
%     (x_u[n],y_u[n]) \leq (L_x,L_y), \forall {n},
% \end{equation}

% where $(L_x,L_y)$ is the maximum 2D coordinates of the area where the simulation scenario is performed. 
% We introduce the peak transmission power $ P_{max}$, where the UL transmission power constraint for the legitimate UE in each time slot is  
% \begin{equation}
%   0 \leq P[n] \leq P_{max}, \forall {n}.
%   \label{11}
% \end{equation}

% The optimization problem of the legitimate capacity $C_{u}$ can now be written as
% \begin{equation}
% \begin{aligned}
%   (P1) : \max\limits_{x_u,y_u,P} \frac{1}{T}\sum\limits_{t=1}^T \Bigg[ %\frac{1}{M}
%      &\log_2 \left( 1+\frac{\zeta_0{P}[t]}{d^2_{u}[t]\sigma^2}\right)%\\
%   %- &\log_2 \left( 1+\frac{\zeta_{0}{P}[t]}{d^{4}_{j}[t]\sigma^2}\right) 
%   \Bigg]%^+
%   ,\\
%   s.t.\hspace{2 pt }(8),(9).
%   \end{aligned}
%   \label{eq:opt_secrecy_rate}
% \end{equation}

% \textcolor{black}{\textbf{Assumptions:}} %List the assumptions that you make or not make as this may be the distinguishing factor or this work w.r.t. others. Justify your assumptions.}
% The following proposed solution for the optimization problem defined in~(\ref{eq:opt_secrecy_rate}) is based on number of assumptions. These assumptions are needed for ensuring the productivity and efficiency of the solution and are described as follows: i) the ABS flies at a constant height that assumed to facilitate the LoS communication with ground users. ii) The location of the passive eavesdropper will be considered as unknown when performing the optimization of the legitimate capacity to provide more practicality for the proposed algorithm. However, the eavesdropper location will only be used for the calculation of secrecy capacity after the end of the optimization scheme.  
